Revisiting constraints on asteroid-mass primordial black holes as dark matter candidates

As the only dark matter candidate that does not invoke a new particle that survives to the present day, primordial black holes (PBHs) have drawn increasing attention recently. Up to now, various observations have strongly constrained most of the mass range for PBHs, leaving only small windows where PBHs could make up a substantial fraction of the dark matter. Here we revisit the PBH constraints for the asteroid-mass window, i.e., the mass range $3.5\times 10^{-17}M_\odot < m_{\mathrm{PBH}} < 4\times 10^{-12}M_\odot$. We revisit 3 categories of constraints. (1) For optical microlensing, we analyze the finite source size and diffractive effects and discuss the scaling relations between the event rate, $m_{\mathrm{PBH}}$ and the event duration. We argue that it will be difficult to push the existing optical microlensing constraints to much lower m$_{\mathrm{PBH}}$. (2) For dynamical capture of PBHs in stars, we derive a general result on the capture rate based on phase space arguments. We argue that survival of stars does not constrain PBHs, but that disruption of stars by captured PBHs should occur and that the asteroid-mass PBH hypothesis could be constrained if we can work out the observational signature of this process. (3) For destruction of white dwarfs by PBHs that pass through the white dwarf without getting gravitationally captured, but which produce a shock that ignites carbon fusion, we perform a 1+1D hydrodynamic simulation to explore the post-shock temperature and relevant timescales, and again we find this constraint to be ineffective. In summary, we find that the asteroid-mass window remains open for PBHs to account for all the dark matter.

==> miscellaneous.tex <==
% === Significant chunks of material that were in the main text, are probably now outdated, but don't want to delete ===

The other way that a long-lived accretion-powered phase of stellar evolution might occur would be if energy injection from accretion puffs up the star and increases $t_{\rm Bondi}$. Note that as the star grows, $\rho \propto R^{-3}$ but $c_s\propto R^{-1/2}$ (via the virial relation), so $t_{\rm Bondi}\propto R^{3/2}$. Since the energy is injected rapidly at the star's center, we should consider the possibility that the star then becomes fully convective and climbs the Hayashi track \cite{1961PASJ...13..450H}.\footnote{This is in some ways similar to what has been proposed for WIMP annihilation-powered stars (e.g., the lower-right panel of Fig.~4 of Ref.~\cite{2009MNRAS.394...82S}).} Since the luminosity on the Hayashi track increases with radius, but the accretion rate onto the central PBH decreases with radius, one might even imagine forming a long-lived luminous giant where the accretion luminosity ($\epsilon\dot m_{\rm PBH} c^2$) equals the luminosity radiated to space, and that might be stable against small perturbations in $R$. To see whether this works, we try setting the luminosity of the star equal to the accretion luminosity at the Bondi rate,
\begin{equation}
4\pi R^2 \sigma T_{\rm eff}^4 = \epsilon \dot m_{\rm PBH} c^2
= \epsilon \frac{4\pi\lambda G^2 \mpbh^2 \rho_{\rm c}}{c_{s,\rm c}^3} c^2,
\end{equation}
where we have take $\rho_{\rm c}$ and the sound speed $c_{s,\rm c}$ to be their values at the center of the star. If we have $\rho_{\rm c} = 1.43 M/R^3$, $c_{s,\rm c} = 0.95 \sqrt{GM/R}$, and $\lambda = 0.25$ -- as appropriate for a $\gamma=\frac53$ polytrope -- then:
% a_1 = 5.991 * 3/(4pi) = 1.43
% a_2 = sqrt(5/3 p_c/rho_c) = 0.95
% (p_c/rho_c = 0.538)
\begin{equation}
R  
= 0.78 \left[ \epsilon \frac{ G^{1/2} c^2 \mpbh^2  }{ \sigma T_{\rm eff}^4 M^{1/2}} \right]^{2/7}
% coef. is (lambda a_1/a_2^3)^{2/7}
= 2\times 10^{13}
\left( \frac{\epsilon}{0.2} \right)^{2/7}
\frac{(\mpbh/10^{-5}\,M_\odot)^{4/7}}{(M/M_\odot)^{1/7}}
\left( \frac{T_{\rm eff}}{3000\,\rm K} \right)^{-8/7}\,{\rm cm}.
\label{eq:R-ultra}
\end{equation}
The numerical value of the temperature is an appropriate for the Hayashi track, which is roughly vertical in the Hertzsprung-Russell diagram due to the steep temperature dependence of H$^-$ opacity. We note that at this stage $\mpbh$ is likely to be at least $M_1$, which from Eq.~(\ref{eq:M1}) would be $1.4\times 10^{-5}(0.2/\epsilon)M_\odot$ for the Sun (hence the chosen scaling). For this reason, reducing $\epsilon$ would actually increase $R$.

In this configuration, the Bondi time is
\begin{eqnarray}
t_{\rm Bondi} &=& \frac{c_{s,\rm c}^3}{4\pi \lambda G^2\mpbh \rho_{\rm c}}
= 0.13 \frac{M^{1/2}}{G^{1/2}\mpbh}\left[ \epsilon \frac{ G^{1/2} c^2 \mpbh^2  }{ \sigma T_{\rm eff}^4 M^{1/2}} \right]^{3/7}
= 0.13 \frac{\epsilon^{3/7} c^{6/7} M^{2/7} }{G^{2/7} \mpbh^{1/7} (\sigma T_{\rm eff}^4)^{3/7} }
\nonumber \\
&=& 4700 \left( \frac{\epsilon}{0.2} \right)^{3/7} 
\frac{(M/M_\odot)^{2/7}}{(\mpbh/10^{-5}\,M_\odot)^{1/7}}
\left( \frac{T_{\rm eff}}{3000\,\rm K} \right)^{-12/7}\,{\rm yr}.
\end{eqnarray}
(If $\mpbh\sim M_1\propto 1/\epsilon$, then the scaling with $\epsilon$ is changed from an exponent of $\frac37$ to $\frac27$, but still it is positive and so lower efficiency reduces $t_{\rm Bondi}$.) Thus it still seems that one might achieve a phase that is long-lived relative to an observational astronomer, though still very short compared to the lifetime of the Universe. (Since the Bondi time decreases only slowly with $\mpbh$ in this scenario, $\propto \mpbh^{-1/7}$, the lifetime obtained by integrating the differential equation for the growth of the PBH is actually $7t_{\rm Bondi}$ -- but see below.)

Several cautions are in order, however. First, even taken at face value, the fiducial estimate of our lifetime is $7t_{\rm Bondi} \sim 33$ kyr; if indeed there have been 4000 capture events in the history of our Galaxy, this suggests that the instantaneous occurrence rate of such stars in a Milky Way-type galaxy is $4000\times (33\,{\rm kyr})/(10\,{\rm Gyr}) \sim 0.01$. In a scenario where PBHs are eating stars and producing such phases, then there should be one accretion-powered giant (which, given the effective temperature and radius, is really only as luminous as some AGB stars) out of the hundred nearest Milky Way-type galaxies. This would be a difficult search, and certainly no published studies rule it out. Second, these accretion-powered giants are subject to a range of potential instabilities. One involves hydrogen recombination: when the interior temperature of a star drops low enough, we must consider partially ionized gas and the $\gamma=\frac53$ polytrope solution is no longer appropriate. More importantly, this may trigger an instability since the adiabatic index of partially ionized gas is $<\frac43$.

This fact about partially ionized stars was recognized in the 1960s during studies of pre-main-sequence evolution \cite{1962Icar....1...13C, 1966ARA&A...4..171H}. In fact, when the energy of ionization (13.6 eV per H atom) is included, stars of sufficiently low central temperature $T_{\rm c}<T_{\rm c,zero}$ have {\em positive} total energy. As the star's radius $R$ grows and $T_{\rm c}$ decreases, there is a temperature $T_{\rm c,max}$ where the energy is maximized (at $E_{\rm max}$), and for even lower $T_{\rm c}$ (larger $R$) the energy decreases. The configurations at $T_{\rm c}$ between $T_{\rm c,max}$ and $T_{\rm c,zero}$ may be stable against adiabatic perturbations, even though diffuse H{\,\sc i} would be a lower energy state. However, if the star reaches $T_{\rm c,max}$, then the addition of any more energy results in no possible hydrostatic solution. The star would be expected to disperse in a hydrogen recombination-powered explosion.

Appendix~\ref{app:Tc} provides the calculation of these temperatures for the idealized case of a pure hydrogen star, including only H{\sc\,i} and H{\sc\,ii} (no H$_2$), with constant entropy per unit mass, and for a total mass of $1\,M_\odot$. This shows that the zero energy crossing occurs at $T_{\rm c} = 95\,000$ K and $R = 8.1\times 10^{12}$ cm; and the maximum occurs at $T_{\rm c} = 37\,000$ K and $R = 2.1\times 10^{14}$ cm. The maximum energy is $E_{\rm max} = 1.2\times 10^{46}$ erg, or 6.0 eV per H atom; we anticipate that this energy would be converted to kinetic energy as the envelope explodes.

It is thus clear that for our fiducial parameters in Eq.~(\ref{eq:R-ultra}), then the hypothesized steady-state accretion-power giant is only an order of magnitude away (in radius) from the stability boundary. Since $R\propto \mpbh^{4/7}$, and the PBH mass evolves as $\mpbh = m_{\rm PBH,0} (1 - t/7t_{\rm Bondi})^7$, the lifetime of the accretion-powered giant may in fact be quite a bit less than $7t_{\rm Bondi}$. Indeed, if $\epsilon\ll 0.2$, then there may not be a stable solution at all. In this case, the star simply proceeds up the Hayashi track and then explodes.

%if a fraction $f$ of the star is consumed during this phase with accretion efficiency $\epsilon$ in time $\Delta t$, then the resulting luminosity is $L = \epsilon fMc^2/\Delta t$.

%We first consider the possibility that the accretion luminosity of the PBH becomes significant and that accretion becomes Eddington rather than Bondi limited. Recall that the characteristic length scale of the accretion flow is set by the Bondi radius $R_{\rm B} = G\mpbh/c_s^2$. The photon mean free path in the ambient medium, if set by Thomson scattering, is $\ell = (\sigma_{\rm T}n_e)^{-1}$. Under conditions at the center of the Sun \cite{2001ApJ...555..990B}, $\ell = 0.024$ cm, which is equal to $R_{\rm B}$ if $\mpbh = m_{\rm PBH,crit} = c_s^2/(G\sigma_{\rm T}n_e) = 4.6\times 10^{-13}\,M_\odot$ (the numerical value is for a PBH captured in the Sun). Thus for $\mpbh \ll m_{\rm PBH,crit}$, the accretion flow is optically thin and for $\mpbh \gg m_{\rm PBH,crit}$ the flow is optically thick. In the optically thin case, we can see that the ratio of the luminosity of Bondi accretion to the Eddington luminosity is
%\begin{eqnarray}
%\frac{L}{L_{\rm Edd}(\mpbh)}
%&=& \frac{\epsilon \dot m_{\rm PBH}c^2}{4\pi Gc \mpbh/\kappa}
%\nonumber \\
%&=& \frac{\epsilon (4\pi \lambda G^2 m_{\rm PBH}^2 \rho/c_s^3)c^2}{4\pi Gc \mpbh/\kappa}
%\nonumber \\
%&=& \frac{\epsilon \lambda G m_{\rm PBH} \rho \kappa c}{ c_s^3}
%\nonumber \\
%&=& \frac{\epsilon \lambda G [c_s^2/(G\sigma_{\rm T}n_e)] n_e\sigma_{\rm T} c}{ c_s^3}
%\frac{m_{\rm PBH}}{m_{\rm PBH,crit}}
%\nonumber \\
%&=& \frac{\epsilon \lambda c}{ c_s}
%\frac{m_{\rm PBH}}{m_{\rm PBH,crit}},
%\end{eqnarray}
%where $\epsilon$ is the radiative efficiency $L/\dot m_{\rm PBH}c^2$. For the solar core, $c/c_s \approx 600$ and $\lambda = 0.25$, and so for low radiative efficiencies ($<0.007$) the accretion flow becomes optically thick before it reaches the Eddington luminosity. For high radiative efficiencies, it is possible that an Eddington-limited phase would occur before the flow becomes optically thick. In any case, for the optically thin phase, the Eddington luminosity $L_{\rm Edd}(\mpbh)$ is very small and not directly observationally significant. If the Eddington time $t_{\rm Edd} = \kappa \epsilon c/(4\pi G)$ is small compared to the lifetime of the star (as it is for the Sun-like case), such a phase would represent only a minor delay before the accretion flow becomes optically thick.

%We should thus consider the behavior of a PBH with an optically thick accretion flow.

%We first consider the proposal that the Bondi accretion phase transitions to an Eddington-limited accretion phase when $t_{\rm Bondi}$ (which is decreasing because it is proportional to $m_{\rm PBH}^{-1}$) reaches $t_{\rm Edd}$ (which depends only on the opacity $\kappa$ and the accretion efficiency $\epsilon = L/\dot m_{\rm PBH}c^2$, where $L$ is the accretion luminosity) \cite{2009arXiv0901.1093R}. Specifically, in Eddington-limited accretion, the PBH mass scales as $\mpbh \propto {\rm e}^{t/t_{\rm Edd}}$, where the Eddington timescale is
%\begin{equation}
%t_{\rm Edd} = \frac{\kappa \epsilon c}{4\pi G}
%= 45\left(\frac{\kappa}{0.4\,{\rm cm}^2\,{\rm g}^{-1}}\right)
%\left( \frac{\epsilon}{0.1} \right)\,{\rm Myr},
%\end{equation}
%where we have scaled $\kappa$ to the pure hydrogen Thomson opacity.

%However, in purely spherical, optically thick accretion, the radiative efficiency $\epsilon$ is negligible: gas is heated as it plunges into the PBH, but the radiation is advected into the hole. Modest $\epsilon$ may occur if the accretion flow is not so optically thick, and some radiation escapes; if the inflowing gas has net angular momentum and hence forms an accretion disc, and then can produce outflows or jets that tap into the gravitational energy released by accretion; or if some instability disrupts the spherical accretion solution and leads to a similar outcome.

%If the duration of such a phase exceeds a few Myr, then we expect at least one such object in the Milky Way right now.

Finally, we need an expression for $dT/dr$, which comes from the condition of constant entropy if the star is assumed to be fully convective. We write
\begin{equation}
\frac{dT}{dr} = \frac TP \frac{dP}{dr} \frac{d\ln T}{d\ln P},
\end{equation}
where $dP/dr$ comes from Eq.~(\ref{eq:dPdr}). The temperature-pressure slope $d\ln T/d\ln P$ is $\frac25$ for a monatomic gas ($\gamma=\frac53$); thus we expect $\frac25$ for both the purely neutral and purely ionized limits. In between, we must do something more sophisticated, using the Saha equation, the ideal gas law, and the first law of thermodynamics. The Saha equation tells us that $2\ln y-\ln(1-y) + \ln \rho  - \frac32\ln T + I_{\rm H}/k_{\rm B}T$ is constant; differentiating this gives
\begin{equation}
\frac{2-y}{y(1-y)}\,dy + d\ln \rho = \left( \frac32 + \frac{I_{\rm H}}{k_{\rm B}T} \right) d\ln T.
\label{eq:B-temp1}
\end{equation}
Differentiation of the ideal gas law, Eq.~(\ref{eq:rho}) gives
\begin{equation}
\frac{dy}{1+y} + d\ln\rho = d\ln P - d\ln T.
\label{eq:B-temp2}
\end{equation}
Finally, we recall the first law of thermodynamics: for zero entropy change, we have $dU + P \, dV = dU - PV\,d\ln\rho = 0$, where $U$ is the energy per unit mass and $V=\rho^{-1} = k_{\rm B}T(1+y)/m_{\rm H}P$ is the volume per unit mass. The energy per unit mass is $U = [\frac32k_{\rm B}T(1+y) + I_{\rm H}y]/m_{\rm H}$. The first law of thermodynamics then gives, after some simplification,
\begin{equation}
\frac32 (1+y) d\ln T + \left( \frac32 + \frac{I_{\rm H}}{k_{\rm B}T} \right) dy  - (1+y) \,d \ln\rho = 0.
\label{eq:B-temp3}
\end{equation}
The combination of Eqs.~(\ref{eq:B-temp1}), (\ref{eq:B-temp2}), and (\ref{eq:B-temp3}) enables us to solve for $d\ln T/d\ln P$:
\begin{equation}
\frac{d\ln T}{d\ln P} = \frac{1 + (\frac 32 + \xi)q}{\frac52 + (\xi^2+5\xi+\frac{15}4)q},
~~~{\rm where}~~~ q = \frac{y(1-y)}{(1+y)(2-y)}~~~{\rm and}~~~
\xi = \frac{I_{\rm H}}{k_{\rm B}T}.
\end{equation}
This completes the needed equations for evolving $T$, $P$, and $m$ (as well as auxiliary variables such as $y$ and $\rho$). Note that $q\rightarrow 0$ for either $y\rightarrow 0$ or $y\rightarrow 1$, and in this case $d\ln T/d\ln P\rightarrow\frac25$; but for partially ionized mixtures and large $\xi$, $d\ln T/d\ln P$ can be very small (but still positive).

In this configuration, the Bondi time is
\begin{eqnarray}
t_{\rm Bondi} &=& \frac{c_{s,\rm c}^3}{4\pi \lambda G^2\mpbh \rho_{\rm c}}
= 0.13 \frac{M^{1/2}}{G^{1/2}\mpbh}\left[ \epsilon \frac{ G^{1/2} c^2 \mpbh^2  }{ \sigma T_{\rm eff}^4 M^{1/2}} \right]^{3/7}
= 0.13 \frac{\epsilon^{3/7} c^{6/7} M^{2/7} }{G^{2/7} \mpbh^{1/7} (\sigma T_{\rm eff}^4)^{3/7} }
\nonumber \\
&=& 4700 \left( \frac{\epsilon}{0.2} \right)^{3/7} 
\frac{(M/M_\odot)^{2/7}}{(\mpbh/10^{-5}\,M_\odot)^{1/7}}
\left( \frac{T_{\rm eff}}{3000\,\rm K} \right)^{-12/7}\,{\rm yr}.
\end{eqnarray}
(If $\mpbh\sim M_1\propto 1/\epsilon$, then the scaling with $\epsilon$ is changed from an exponent of $\frac37$ to $\frac27$, but still it is positive and so lower efficiency reduces $t_{\rm Bondi}$.) Thus it still seems that one might achieve a phase that is long-lived relative to an observational astronomer, though still very short compared to the lifetime of the Universe. (Since the Bondi time decreases only slowly with $\mpbh$ in this scenario, $\propto \mpbh^{-1/7}$, the lifetime obtained by integrating the differential equation for the growth of the PBH is actually $7t_{\rm Bondi}$ -- but see below.)

Several cautions are in order, however. First, even taken at face value, the fiducial estimate of our lifetime is $7t_{\rm Bondi} \sim 33$ kyr; if indeed there have been 4000 capture events in the history of our Galaxy, this suggests that the instantaneous occurrence rate of such stars in a Milky Way-type galaxy is $4000\times (33\,{\rm kyr})/(10\,{\rm Gyr}) \sim 0.01$. In a scenario where PBHs are eating stars and producing such phases, then there should be one accretion-powered giant (which, given the effective temperature and radius, is really only as luminous as some AGB stars) out of the hundred nearest Milky Way-type galaxies. This would be a difficult search, and certainly no published studies rule it out. Second, these accretion-powered giants are subject to a range of potential instabilities. 

It is thus clear that for our fiducial parameters in Eq.~(\ref{eq:R-ultra}), then the hypothesized steady-state accretion-power giant is only an order of magnitude away (in radius) from the stability boundary. Since $R\propto \mpbh^{4/7}$, and the PBH mass evolves as $\mpbh = m_{\rm PBH,0} (1 - t/7t_{\rm Bondi})^7$, the lifetime of the accretion-powered giant may in fact be quite a bit less than $7t_{\rm Bondi}$. Indeed, if $\epsilon\ll 0.2$, then there may not be a stable solution at all. In this case, the star simply proceeds up the Hayashi track and then explodes.

\chris{[really need to add He into this calculation before we submit this, it will probably destabilize even stars that are more compact. also the scale height is so enormous if we really have $R>10^{14}$ cm that the outer boundary condition may not make much sense anymore.]}

We conclude that capture of a PBH may or may not lead to an accretion-powered giant phase (a definitive calculation would be very difficult), and even if this phase does occur, its short lifetime means that these stars would be rare ($<0.01$ per Milky Way-type galaxy) and difficult to detect.


